On in-silico estimation of left ventricular end-diastolic pressure from cardiac strains

Left ventricular diastolic dysfunction (LVDD) is a group of diseases that adversely affect the passive phase of the cardiac cycle and can lead to heart failure. While left ventricular end-diastolic pressure (LVEDP) is a valuable prognostic measure in LVDD patients, traditional invasive methods of measuring LVEDP present risks and limitations, highlighting the need for alternative approaches. This paper investigates the possibility of measuring LVEDP non-invasively using inverse in-silico modeling. We propose the adoption of patient-specific cardiac modeling and simulation to estimate LVEDP and myocardial stiffness from cardiac strains. We have developed a high-fidelity patient-specific computational model of the left ventricle. Through an inverse modeling approach, myocardial stiffness and LVEDP were accurately estimated from cardiac strains that can be acquired from in vivo imaging, indicating the feasibility of computational modeling to augment current approaches in the measurement of ventricular pressure. Integration of such computational platforms into clinical practice holds promise for early detection and comprehensive assessment of LVDD with reduced risk for patients.

==> bib.tex <==
@article{Guccione1991,
	title={Passive material properties of intact ventricular myocardium determined from a cylindrical model},
	author={Guccione, J.M. and McCulloch, A.D. and Waldman, L.K.},
	journal={J. Biomech. Eng.},
	volume={113},
	number={1},
	pages={42--55},
	year={1991},
	publisher={American Society of Mechanical Engineers}
}

@article{Mendiola2024,
title = {An image-driven micromechanical approach to characterize multiscale remodeling in infarcted myocardium},
journal = {Acta Biomaterialia},
volume = {173},
pages = {109-122},
year = {2024},
issn = {1742-7061},
doi = {https://doi.org/10.1016/j.actbio.2023.10.027},
url = {https://www.sciencedirect.com/science/article/pii/S1742706123006359},
author = {Emilio A. Mendiola and Sunder Neelakantan and Qian Xiang and Shuda Xia and Jianyi Zhang and Vahid Serpooshan and Peter Vanderslice and Reza Avazmohammadi},
keywords = {Myocardial infarction, In-silico modeling, Multiscale remodeling, Cardiac strains, Scar maturation},
abstract = {Myocardial infarction (MI) is accompanied by the formation of a fibrotic scar in the left ventricle (LV) and initiates significant alterations in the architecture and constituents of the LV free wall (LVFW). Previous studies have shown that LV adaptation is highly individual, indicating that the identification of remodeling mechanisms post-MI demands a fully subject-specific approach that can integrate a host of structural alterations at the fiber-level to changes in bulk biomechanical adaptation at the tissue-level. We present an image-driven micromechanical approach to characterize remodeling, assimilating new biaxial mechanical data, histological studies, and digital image correlation data within an in-silico framework to elucidate the fiber-level remodeling mechanisms that drive tissue-level adaptation for each subject. We found that a progressively diffused collagen fiber structure combined with similarly disorganized myofiber architecture in the healthy region leads to the loss of LVFW anisotropy post-MI, offering an important tissue-level hallmark for LV maladaptation. In contrast, our results suggest that reductions in collagen undulation are an adaptive mechanism competing against LVFW thinning. Additionally, we show that the inclusion of subject-specific geometry when modeling myocardial tissue is essential for accurate prediction of tissue kinematics. Our approach serves as an essential step toward identifying fiber-level remodeling indices that govern the transition of MI to systolic heart failure. These indices complement the traditional, organ-level measures of LV anatomy and function that often fall short of early prognostication of heart failure in MI. In addition, our approach offers an integrated methodology to advance the design of personalized interventions, such as hydrogel injection, to reinforce and suppress native adaptive and maladaptive mechanisms, respectively, to prevent the transition of MI to heart failure.
Statement of significance
Biomechanical and architectural adaptation of the LVFW remains a central, yet overlooked, remodeling process post-MI. Our study indicates the biomechanical adaptation of the LVFW post-MI is highly individual and driven by altered fiber network architecture and collective changes in collagen fiber content, undulation, and stiffness. Our findings demonstrate the possibility of using cardiac strains to infer such fiber-level remodeling events through in-silico modeling, paving the way for in-vivo characterization of multiscale biomechanical indices in humans. Such indices will complement the traditional, organ-level measures of LV anatomy and function that often fall short of early prognostication of heart failure in MI.}
}

@InProceedings{Usman2023,
author="Usman, Muhammad
and Mendiola, Emilio A.
and Mukherjee, Tanmay
and Mehdi, Rana Raza
and Ohayon, Jacques
and Alluri, Prasanna G.
and Sadayappan, Sakthivel
and Choudhary, Gaurav
and Avazmohammadi, Reza",
editor="Bernard, Olivier
and Clarysse, Patrick
and Duchateau, Nicolas
and Ohayon, Jacques
and Viallon, Magalie",
title="On the Possibility of Estimating Myocardial Fiber Architecture from Cardiac Strains",
booktitle="Functional Imaging and Modeling of the Heart",
year="2023",
publisher="Springer Nature Switzerland",
address="Cham",
pages="74--83",
abstract="The myocardium is composed of a complex network of contractile myofibers that are organized in such a way as to produce efficient contraction and relaxation of the heart. The myofiber architecture in the myocardium is a key determinant of cardiac motion and the global or organ-level function of the heart. Reports of architectural remodeling in cardiac diseases, such as pulmonary hypertension and myocardial infarction, potentially contributing to cardiac dysfunction call for the inclusion of an architectural marker for an improved assessment of cardiac function. However, the in-vivo quantification of three-dimensional myo-architecture has proven challenging. In this work, we examine the sensitivity of cardiac strains to varying myofiber orientation using a multiscale finite-element model of the LV. Additionally, we present an inverse modeling approach to predict the myocardium fiber structure from cardiac strains. Our results indicate a strong correlation between fiber orientation and LV kinematics, corroborating that the fiber structure is a principal determinant of LV contractile behavior. Our inverse model was capable of accurately predicting the myocardial fiber range and regional fiber angles from strain measures. A concrete understanding of the link between LV myofiber structure and motion, and the development of non-invasive and feasible means of characterizing the myocardium architecture is expected to lead to advanced LV functional metrics and improved prognostic assessment of structural heart disease.",
isbn="978-3-031-35302-4"
}

@article{Avazmohammadi2019a,
    author = {Avazmohammadi, R and Mendiola, E A and Soares, J S and Li, D S and Chen, Z and Merchant, S and Hsu, E W and Vanderslice, P and Dixon, RAF and Sacks, MS},
    title = "{A Computational Cardiac Model for the Adaptation to Pulmonary Arterial Hypertension in the Rat}",
    journal = {Annals of Biomedical Engineering},
    volume = {47},
    number = {1},
    pages = {138-153},
    year = {2019},
    month = {09},
    issn = {0008-6363},
    doi = {10.1007/s10439-018-02130-y},
}
